Cohorting to isolate asymptomatic spreaders: An agent-based simulation study on the Mumbai Suburban Railway

The Mumbai Suburban Railways, \emph{locals}, are a key transit infrastructure of the city and is crucial for resuming normal economic activity. To reduce disease transmission, policymakers can enforce reduced crowding and mandate wearing of masks. \emph{Cohorting} -- forming groups of travelers that always travel together, is an additional policy to reduce disease transmission on \textit{locals} without severe restrictions. Cohorting allows us to: ($i$) form traveler bubbles, thereby decreasing the number of distinct interactions over time; ($ii$) potentially quarantine an entire cohort if a single case is detected, making contact tracing more efficient, and ($iii$) target cohorts for testing and early detection of symptomatic as well as asymptomatic cases. Studying impact of cohorts using compartmental models is challenging because of the ensuing representational complexity. Agent-based models provide a natural way to represent cohorts along with the representation of the cohort members with the larger social network. This paper describes a novel multi-scale agent-based model to study the impact of cohorting strategies on COVID-19 dynamics in Mumbai. We achieve this by modeling the Mumbai urban region using a detailed agent-based model comprising of 12.4 million agents. Individual cohorts and their inter-cohort interactions as they travel on locals are modeled using local mean field approximations. The resulting multi-scale model in conjunction with a detailed disease transmission and intervention simulator is used to assess various cohorting strategies. The results provide a quantitative trade-off between cohort size and its impact on disease dynamics and well being. The results show that cohorts can provide significant benefit in terms of reduced transmission without significantly impacting ridership and or economic \& social activity.

==> datasets.tex <==
% \section{Simulation Datasets}
% We digitized the \href{https://upload.wikimedia.org/wikipedia/commons/thumb/7/78/Mumbai_Rail_Map_-_English.jpg/1280px-Mumbai_Rail_Map_-_English.jpg}{Mumbai Rail Map}, and capture train line, train station, transit time between consecutive stations along a line, along with station latitude, longitude information. We restrict ourselves to the census city limits of Mumbai and Mumbai suburbs, to be consistent with agents being generated, and have 52 stations in the network. This data is used to pre-compute shortest travel route and corresponding time between any two stations across any line, making heuristic assumptions of transition time when the journey consists of multiple legs.

% 2011-12 Census for Mumbai and Mumbai suburbs provides demographic information around age, gender, households at Ward level (overall 24 wards). Workplaces and schools are assigned heuristically, mapping students to schools in the same ward. For travel between home and workplace we optimize for travel time across various modes of travel, accounting for frequency and cost differential of road commute options compared to using \emph{locals}, the expected speed of travel via road (21.6 km/h) and geodesic to road detour index, and also consider multiple possible train stations an agent would consider as the primary commute stations both for home and workplace location. This overall allows us to know which agents take trains, and what route they follow. During the simulation we use this information for forming cohorts, as well as evaluating travel overlap time between different agents based on their co-occupancy of a train coach for disease transmission.

